Semantic Change and Emerging Tropes In a Large Corpus of New High German Poetry

Due to its semantic succinctness and novelty of expression, poetry is a great test bed for semantic change analysis. However, so far there is a scarcity of large diachronic corpora. Here, we provide a large corpus of German poetry which consists of about 75k poems with more than 11 million tokens, with poems ranging from the 16th to early 20th century. We then track semantic change in this corpus by investigating the rise of tropes (`love is magic') over time and detecting change points of meaning, which we find to occur particularly within the German Romantic period. Additionally, through self-similarity, we reconstruct literary periods and find evidence that the law of linear semantic change also applies to poetry.

==> 07_ToDoList.tex <==
\section*{Paper to do list:}

============================================================================ 
LChange' 19 Reviews for Submission #49
============================================================================ 
 
Title: Semantic Change and Emerging Tropes In a Large Corpus of New High German Poetry
Authors: Thomas Haider and Steffen Eger
============================================================================
                            REVIEWER #1
============================================================================
 
---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                   Appropriateness (1-5): 5
                           Clarity (1-5): 2
      Originality / Innovativeness (1-5): 4
           Soundness / Correctness (1-5): 4
                    Recommendation (1-5): 3
 
Detailed Comments
---------------------------------------------------------------------------
>>The paper needs more detailed explanations and a better presentation and a more logical structure to be easily understandable.
 -- MORE DETAILED EXPLANATIONS, BETTER PRESENTATION, LOGICAL STRUCTURE
 
>>I am not sure why the abstract does not mention the experiments of self-similarity. If it's important enough to be half of the experiments, it should be there.
 -- ABSTRACT
 
What are the percentiles represented by the whiskers in the box plot in Figure 2?
 whis : float, sequence, or string (default = 1.5)
As a float, determines the reach of the whiskers to the beyond the first and third quartiles. In other words, where IQR is the interquartile range (Q3-Q1), the upper whisker will extend to last datum less than Q3 + whis*IQR). Similarly, the lower whisker will extend to the first datum greater than Q1 - whis*IQR. Beyond the whiskers, data are considered outliers and are plotted as individual points. Set this to an unreasonably high value to force the whiskers to show the min and max values. Alternatively, set this to an ascending sequence of percentile (e.g., [5, 95]) to set the whiskers at specific percentiles of the data. Finally, whis can be the string 'range' to force the whiskers to the min and max of the data.
 
 
The structure of the Experiment section is not clear.
    -- OK?
 
The self-similarity sections would benefit from pseudocode clarifying the underlying algorithms. 
    -- PSEUDOCODE?
 
Wouldn't the experiment in Pairwise Self-Similarity require an alignment (rotation) of the embeddings calculated at every time period? The embeddings in different spaces cannot be compared directly, it's their relative positions what matters.
 -- ??? That's what the joint model is for.
 
Figure 5 is needing more explanation: axes, what the different types of line mean, etc. It's not enough if it comes up later on in the running text.
 -- Trajectory expanation not in running text, but in caption
 
 
In Section "Emerging Tropes: Collocations & Metaphors Method", how the high dimensional space is built needs to be explained more formally.
-- High Dimensional Space? How to build a PCA of trajectories?
 
Overlapping labels in Figure 4 need to be resolved in some way.
-- I WISH
 
The translations to English would be better in the running text, or perhaps even better in a table, rather than in footnotes that require the reader go back and forth numerous times.
-- Period translations in running text
 
Minor language issues:
In Section "Pairwise Self-Similarity"
- Missing space: "the cosine similarityof the "
- Typo "analyis."
---------------------------------------------------------------------------
 
 
 
============================================================================
                            REVIEWER #2
============================================================================
 
---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                   Appropriateness (1-5): 5
                           Clarity (1-5): 3
      Originality / Innovativeness (1-5): 3
           Soundness / Correctness (1-5): 4
                    Recommendation (1-5): 3
 
Detailed Comments
---------------------------------------------------------------------------
Summary:
 
Semantic change occurs gradually in language but is often difficult to detect. The study proposes an analysis of semantic change in German poetry, focusing on specific poetic tropes such as "love." 
/// Love is not a Trope /// 
It is shown that word semantics were "homogenized" in the middle of the poetic period, 
/// WHAT? ??? /// 
that high-frequency words have lower self-similarity over time, and that the words associated with the word "love" follow several prominent trends in change trajectories (e.g. "falling" similarity). 
/// Can be shown for all word pairs ///
 
Strengths:
- Provides a simple yet effective extension of a previous method for word embedding customization.
- Tests a hypothesis related to frequency and semantic change and finds evidence to question prior findings.
- Detects changes in common tropes associated with romantic poetry, which provides further insight for literary scholars to investigate. This type of analysis seems novel and worth more exploration, such as formulating a general method for detecting the emergence or loss of trope types in poetry. /// What would be a more general method? ///
 
Weaknesses:
- Basic model details are missing and make it hard to judge the paper. How many dimensions were used, what algorithm (word2vec?) /// Yes /// 
was used to train the embeddings, do the resulting embeddings have reasonable properties (e.g. logical nearest neighbors)? 
/// Yes. Showing KNNs? ///

- The study needs better justification in the introduction. What kinds of questions about poetry can we answer by studying semantic change? 
/// Good point ///

- The analysis of self-similarity is not too convincing, because of details omitted and overall research questions. For instance, did the "homogenization" finding correlate with prevailing literary theories? 
/// Yes, but that needs space /// 

Are there any words that are good examples of the homogenization trend (e.g. "love" often used in the same context in the 1750 time bin)? 
/// Could be tested, but how, if not by cossim? /// 

Was the finding robust across different subsets of the vocabulary (top-100, top-500, etc.)? 
/// Yes, more or less /// 

- The analysis of emerging tropes is difficult to interpret because of the small and unreadable graphs (Figures 4 and 5). It would be better to split Figure 5 into 4 separate sub-plots for the different trend types. 
/// So four graphs for trajectories /// 
 
Comments:
- Line 42 "which allows (them)"
- Inconsistent capitalization of time periods ("barock" vs. "Barock").


\begin{todolist}
    % \item[\done] Play with LEGO
    % \item[\done] Acknowledgements
    % \item[\done] Author contributions
    % \item[\done] Handle how Dix paper is introduced
    % \item[\done] Move Event detection dataset to main text (?)
    % \item Check video links
    % \item Check link and completeness of software/hardware availability
    % \item Check list of references
    % \item Complete Materials and methods
    % \item[\done] Add Christophe's reference to the bibliography
    % \item consider merging main text and methods bibliography(?)
    % \item[\done] Decide whether to include the dual color imaging with CD4/actin or not
    % \item[\done] Tidy up SuppInfo
    % \item dSTORM to STORM in SuppInfo + Movies
    
    \item[\done] Write abstract (RFL, RH)
    \item Obtain data for figures and design figures (KT)
    
    
The aim of this workshop is three-fold. First, we want to provide pioneering researchers who work on computational methods, evaluation, and large-scale modelling of language change an outlet for disseminating cutting-edge research on topics concerning language change. Currently, researchers in this area have published in a wide range of different venues, from computational linguistics, to cognitive science and digital archiving venues. We want to utilize this proposed workshop as a platform for sharing state-of-the-art research progress in this fundamental domain of natural language research.

Second, in doing so we want to bring together domain experts across disciplines. We want to connect those that have long worked on language change within historical linguistics and bring with them a large understanding for general linguistic theories of language change; those that have studied change across languages and language families; those that develop and test computational methods for detecting semantic change and laws of semantic change; and those that need knowledge (of the occurrence and shape) of language change, for example, in digital humanities and computational social sciences where text mining is applied to diachronic corpora subject to lexical semantic change.

Third, the detection and modelling of language change using diachronic text and text mining raise fundamental theoretical and methodological challenges for future research in this area. The representativeness of text is a first critical issue; works using large diachronic corpora and computational methods for detecting change often claim to find changes that are universally true for a language as a whole. But the jury is out on how results derived from digital literature or newspapers accurately represent changes in language as a whole. We hope to engage corpus linguists, big-data scientists, and computational linguists to address these open issues. Besides these goals, this workshop will also support discussion on the evaluation of computational methodologies for uncovering language change. Verifying change only using positive examples of change often confirms a corpus bias rather than reflecting genuine language change. Larger quantities and higher qualities of text over time result in the detection of more semantic change. In fact, multiple semantic laws have been proposed lately where later other authors have shown that the detected effects are linked to frequency rather than underlying semantic change . The methodological issue of evaluation, together with good evaluation testsets and standards are of high importance to the research community. We aim to shed some light on these issues and encourage the community to collaborate to find solutions.

We invite original research papers from a wide range of topics, including but not limited to:

Automatic detection of semantic change and diachronic lexical replacement
Fundamental laws of language change
Computational theories and generative models of language change
Sense-aware (semantic) change analysis
Methodologies for resource-poor languages
Diachronic linguistic data visualization and online systems
Applications and implications of language change detection
Sociocultural influences on language change
Cross-linguistic and phylogenetic approaches to language change
Methodological aspects of, as well as datasets for, evaluation
The workshop is planned to last a full day. Submissions are open to all, and are to be submitted anonymously. All papers will be refereed through a double-blind peer review process by at least three reviewers with final acceptance decisions made by the workshop organizers. We plan to edit a book on the basis of extended workshop papers and are currently discussing the publication with a publisher.
  
   A move towards multi-sense embeddings will most likely require even more texts per time unit, which will limit the applicability of these methods to other languages than English and a few others. We want to bring about a discussion on the need for methods that can discriminate and disambiguate among a word's senses (meanings) and that can be used for resource-poor languages with little hope of acquiring the order of magnitude of words needed for creating stable embeddings, possibly using dynamic embeddings that seem to require less text . Finally, knowledge of language change is useful not only on its own, but as a basis for other diachronic textual investigations and in search.
   
    By reaching out to these other communities, we can better understand how to utilize the results for further research and for presenting them to the interested public. In addition, we need good user interfaces and systems for exploring language changes in corpora, for example, to allow for serendipitous discovery of interesting phenomena . In addition to facilitate research on texts, information about language changes is used for measuring document across-time similarity, information retrieval from long-term document archives, the design of OCR algorithms and so on.


\end{todolist}




==> WordCount.tex <==
\section*{Word Counts}
This section is \textit{not} included in the word count.



\subsection*{Notes on JPhysD article}
\begin{itemize}
    \item Abstract: 150 words, unreferenced
    % \item Sections: Introduction Results, Discussion, Online Methods. Topical subheadings allowed in Results and Online Methods
    \item Main text: short format 4500 words, long is 8500 words.
    \item No limit in number of figures
    % \item References: Up to 40
\end{itemize}

\section*{Statistics on word count}

\immediate\write18{texcount -utf8 -nobib -merge -sum -dir 01_Article_MainText.tex > \jobname.wcdetail }
\verbatiminput{\jobname.wcdetail}

